Tree-structured Policy Planning with Learned Behavior Models

Autonomous vehicles (AVs) need to reason about the multimodal behavior of neighboring agents while planning their own motion. Many existing trajectory planners seek a single trajectory that performs well under \emph{all} plausible futures simultaneously, ignoring bi-directional interactions and thus leading to overly conservative plans. Policy planning, whereby the ego agent plans a policy that reacts to the environment's multimodal behavior, is a promising direction as it can account for the action-reaction interactions between the AV and the environment. However, most existing policy planners do not scale to the complexity of real autonomous vehicle applications: they are either not compatible with modern deep learning prediction models, not interpretable, or not able to generate high quality trajectories. To fill this gap, we propose Tree Policy Planning (TPP), a policy planner that is compatible with state-of-the-art deep learning prediction models, generates multistage motion plans, and accounts for the influence of ego agent on the environment behavior. The key idea of TPP is to reduce the continuous optimization problem into a tractable discrete Markov Decision Process (MDP) through the construction of two tree structures: an ego trajectory tree for ego trajectory options, and a scenario tree for multi-modal ego-conditioned environment predictions. We demonstrate the efficacy of TPP in closed-loop simulations based on real-world nuScenes dataset and results show that TPP scales to realistic AV scenarios and significantly outperforms non-policy baselines.

==> [Chen.ea.ICRA.22]Contingency planning/approach_full.tex <==
\section{Tree Policy Planning}\label{sec:formulation}

\algname{} generates the ego motion policy in three steps as shown in Fig.~\ref{fig:diagram}. First, the ego motion sampler generates an \emph{ego trajectory tree}, $\bfr$, given the current ego state and a lane map (when available). The ego trajectory tree consists of connected, dynamically feasible trajectory segments that together represent candidate ego-vehicle trajectories the planner can choose from. Second, the prediction module is a deep learned model that generates multi-modal predictions of the environment in the form of a \emph{scenario tree}, $\bfe$. % We experiment with three different deep learning models for prediction that can optionally be conditioned on hypothetical ego trajectories during planning. 
Finally, the dynamic programming module % contingency planner 
converts $\bfr$ and $\bfe$ into an MDP and finds an optimal policy via dynamic programming. 

% Before diving into the methodology, we review some key notations. 
We use the following notation. Let $s_r$ denote the state of the ego vehicle and $s_e$ denote the state of the environment, including the state of nearby agents and the location of static obstacles. %The two critical concepts, trajectory tree and scenario tree, are tree structures with branches containing segments of trajectories. 
For the trajectory tree, $r^i_j$ denotes the $j$-th node of stage $i$ and and the root node is simply $r^0$. The nodes in the scenario tree are labeled the same way. We enforce that all nodes of the same stage contain trajectories of the same duration with $t^i_0$ and $t_f^i$ being the starting and ending time of the $i$-th stage. The trajectory of a any node other than the root needs to follow the trajectory of its parent node. For both trees, $\pa(\cdot)$ denotes the parent of a node and $\ch(\cdot)$ denote the set of children of a node, e.g., $\pa(r_1^1)=r^0$, $\ch(e_0^1)=\{e^2_0,e^2_1\}$ for the two trees in Fig. \ref{fig:diagram}. 
%Sometimes with a slight abuse of notation, we use $\ch(\cdot)$ to denote the set of indices of the children branches. 

% \begin{figure}%
%     \centering
%     \subfloat[\centering Trajectory tree]{{\includegraphics[width=0.4\columnwidth]{traj_tree.png} }}%
%     \qquad
%     \subfloat[\centering Scenario tree]{{\includegraphics[width=0.4\columnwidth]{scenario_tree.png} }}%
%     \caption{Example trajectory tree and scenario tree with labels}%
%     \label{fig:tree}
%     \vspace{-0.5cm}
% \end{figure}


Next, we discuss the three components in detail.



%%%%%%%%%%%%

% \section{Tree Policy Planning}\label{sec:overview}

% \comment{this is an alternatively organization of the content in sec: problem formulation}

% We begin with a high-level overview of our Tree Policy Planning algorithm and introduce some important notation.  

% The \algname{} algorithm is shown in Fig.~\ref{fig:diagram}. It generates a contingent ego motion policy in three steps. First, the ego motion sampler generates an \emph{ego trajectory tree}, $\bfr$. The ego trajectory tree consists of connected, dynamically feasible  trajectory segments that together represent possible ego-vehicle trajectories the planner can choose from. \TODO{short sentence on the module}
% Second, the prediction module generates a \emph{scenario tree}, $\bfe$. The scenario tree predicts the environment behavior within the planning horizon for all visible traffic agents. The scenario tree can potentially depend on the ego trajectory tree if ego-conditioning is enabled.  \TODO{short sentence on the module}
% Third, given $\bfr$ and $\bfe$, the contingency planner generates the optimal motion policy via dynamic programming.  \TODO{short sentence on the module} 

% More formally, we let $s_r$ denote the state of the ego vehicle and $s_e$ denote the state of the environment, including the state of nearby agents and the location of static obstacles. The trajectory tree represents the possible motions of the ego vehicle, where $r^i_j$ denotes the $j$-th branch of stage $i$ and and the root branch is simply $r^0$. We enforce that all branches of the same stage contain trajectories of the same duration with $t^i_0$ and $t_f^i$ being the starting and ending time of the $i$-th stage. The trajectory of a any branch other than the root needs to follow the trajectory of its parent branch.

% Similarly, a scenario tree contains trajectory predictions of the nearby agents and is synchronized with the trajectory tree, i.e., the starting and ending time of its branches are consistent with the trajectory tree. The branching is caused by multimodal predictions from the prediction model. We let $e^i_j$ denote the $j$-th branch in the $i$-th stage of the scenario tree. For both trees, $\pa(\cdot)$ denotes the parent of a branch and $\ch(\cdot)$ denote the set of children of a branch, e.g., $\pa(r_1^1)=r^0$, $\ch(e_0^1)=\{e^2_0,e^2_1\}$ for the two trees in Fig. \ref{fig:diagram}. 

% Next, we discuss the three components in detail.





\subsection{Ego-motion sampler}\label{sec:sampler}
The ego motion sampler generates a set of dynamically feasible trajectory options for planning to consider, and organizes them into a trajectory tree. 

\noindent\myparagraph{Terminal point sampling.} We first sample a set of terminal points and then find a feasible trajectory to the terminal point.
Terminal points are sampled from a fixed set of acceleration-steering values, as well as along (and near to) lane centerlines when lane information is available. 

\noindent\myparagraph{Spline fitting.} We then fit a spline from the current ego state to the terminal point following \cite{schmerling2018multimodal}.
% Specifically, the ego vehicle's dynamics is modeled as a unicycle with
% \begin{equation}\label{eq:unicycle}
%     s_r=\begin{bmatrix}X&Y&v&\psi\end{bmatrix}^\intercal,\; \dot{s}_r=\begin{bmatrix}v \cos\psi&v\sin\psi&a&\dot{\psi} \end{bmatrix}^\intercal
% \end{equation}
% where the four states are $X,Y$ positions, velocity, and heading angle, and the inputs are acceleration $a$ and yaw rate $\dot{\psi}$.
\comment{the rest can be removed if needed}
Given the current ego state $s_r[0]=[X_0,Y_0,v_0,\psi_0]^\intercal$ and a terminal condition $s_r[T]=[X_T,Y_T,v_T,\psi_T]^\intercal$, we use two separate polynomials $X[t]$ and $Y[t]$ to parameterize the $X,Y$ coordinates such that the resulting spline connects the two points and the boundary conditions are met:
\begin{equation}
\begin{aligned}
    X[0]&=X_0\quad &X[T]&=X_T\\
    Y[0]&=Y_0\quad &Y[T]&=Y_T\\
    \dot{X}[0]&=v_0 \cos\psi_0\quad &\dot{X}[T]&=v_T \cos\psi_T\\
    \dot{X}[0]&=v_0 \sin\psi_0\quad &\dot{X}[T]&=v_T \sin\psi_T.
\end{aligned}
\end{equation}
With four boundary conditions on each polynomial, two 3rd order (cubic) polynomial can be uniquely determined, which allows us to directly compute the coefficient of $X[t]$ and $Y[t]$ in closed-form and calculate the trajectory from $X[t]$ and $Y[t]$. 
Finally we drop trajectories that violate dynamic constraints. 

\noindent\myparagraph{Tree construction.} In practice, trajectory trees are grown stage by stage, starting from the current state as root $r^0$. We set an upper bound on the number of children a node can have, and randomly drop children nodes if the limit is exceeded. % During sampling, the lane-dependent terminal points are prioritized. 
In each stage we grow children branches in parallel, thus the time complexity is linear in stage number.


\subsection{Multi-stage prediction model}\label{sec:pred}
A critical part of \algname{} is the prediction model that generates a scenario tree. For policy planning, we need a scene-centric, ego-conditioned, and multi-stage prediction model. We will first review these requirements and then show examples of deep-learning models satisfying our requirements.

\noindent\myparagraph{Requirements.} 
First, the prediction model needs to predict \emph{multiple modes} of the trajectory distribution for each agent. Second,  predictions must be \textit{scene-centric}, i.e., outputting modes of the joint trajectory distribution of all relevant agents in the scene. Branches of our scenario tree corresponds to modes of the joint distribution so that our planner will be able to evaluate ego trajectory candidates against joint futures effectively. Examples for multi-modal scene-scentric predictions include~\cite{agentformer,ScePT}.
Third, we need \textit{ego-conditioning} (EC), i.e., prediction results should be conditioned on the ego vehicle's hypothetical future motion. Ego conditioning allows the planner to leverage the reactive behaviors of the environment towards the ego vehicle and is a known technique in prediction literature \cite{T++,ScePT}. However, training a EC prediction model remains challenging as the ground truth under counterfactual ego future motion is not known.

Lastly, we need to generate modes of the predicted trajectory distribution in \emph{multiple stages}. That is, the generated scenario tree contains multiple stages with each node branching into multiple children after each stage. Multistage prediction allows the ego agent to depend its future motion on the future multimodal observation of the environment (similar to a decision tree) and the stage number can be freely set as a design choice. Details on converting existing models to enable multistage prediction can be found in the appendix.

\noindent\myparagraph{Model architectures.} To evaluate \algname{}'s flexibility w.r.t. different prediction models, we tested it with three vastly distinct prediction models. The first model is a rasterized model with CNN backbone and a CVAE; the second model is the PredictionNet \cite{predictionnet} model with a Unet backbone, and the third model is the Agentformer model \cite{agentformer}. All models are modified to enable multistage prediction and ego-conditioning. Details can be found in the appendix. 

% Most existing contingency planning works with a multimodal setup \cite{hardy2013contingency,cui2021lookout} only perform the mode enumeration once, i.e., the ego vehicle identifies which mode the environment is in and executes the corresponding plan. We advocate for a multistage prediction model, which allows the contingency planner to adjust the ego plan at each branching point, thus greatly enlarges the space of possible policies for the ego vehicle. Recall the example in Fig. \ref{fig:diagram}, with a single stage, the ego vehicle needs to identify whether the red vehicle is changing lane immediately after planning while using multiple stages allows the ego vehicle to rely on future observations down the horizon and hedge its current motion on possible future events. We follow \cite{chen2022interactive} and construct a scenario tree for multistage contingency planning. We shall later show three examples where existing prediction models are extended to generate \textit{multistage} predictions. 

% One underlying requirement is that the prediction module needs to be \textit{scene-centric}, i.e., jointly predicting trajectories of all relevant agents in the scene. This is because the ego trajectory candidates are evaluated against all agents' trajectories in the scene, and each branch of the scenario tree corresponds to a mode of the joint prediction.

% \textit{Ego-conditioning} means that the prediction result depends on the ego vehicle's hypothetical future motion. Ego conditioning allows the planner to leverage the reactive behaviors of the environment towards the ego vehicle and is a known technique in prediction/planning literature \cite{T++,ScePT}. \cite{chen2022interactive} uses a differentiable ego-conditioned model and optimizes the ego plan and the environment's reaction together via gradient-based optimization; \cite{fisac2019hierarchical} let the inner loop generate the environment's reaction to the ego and the outer loop to optimize over the ego plan via dynamic programming. For a sampling-based planner, the candidate ego trajectories are known and can be directly fed to the prediction model. Since no gradient is needed, powerful deep-learning models can be leveraged. However, training a ego-conditioned prediction model remains challenging as the ground truth under counterfactual ego future motion is not known.

% To evaluate \algname{}'s flexibility and sensitivity over different prediction models, we tested it with three vastly distinct prediction models. The first model is a rasterized model with CNN backbone and a CVAE; the second model is the PredictionNet \cite{predictionnet} model with a Unet backbone, and the third model is the Agentformer model \cite{agentformer}. All models are modified to enable multistage prediction and ego-conditioning. The details can be found in the appendix.





% \begin{remark}
% The reason for not using re-rasterization for the CNN-based model is that its rasterized feature is centered around each agent, which requires cropping and rotating the map and then paint the boxes, which is more expensive than simply updating the boxes.
% \end{remark}


\subsection{Dynamic programming}\label{sec:DP}
The dynamic programming module takes the ego trajectory tree $\bfr$ and the scenario tree $\bfe$, along with a handcrafted cost function $l$ and finds an optimal ego motion policy. 

Intuitively, our algorithm constructs a discrete MDP over $\bfr$ and $\bfe$ and finds an optimal policy through dynamic programming. More specifically, states of the MDP are nodes %branches 
of the scenario/trajectory trees that represent the joint ego and environment state; transitions are given by the tree parent/children edges in the two trees; and rewards are defined by the integral of the cost over the time segment. We then solve for the optimal finite-horizon \emph{policy} for the discrete MDP using dynamic programming, i.e., calculating the value function backwards in stage via the Bellman equation. With the optimal policy, the continuous-time trajectory is recovered from the trajectory tree by executing the trajectory segments according to the policy. In practice we use a cost function $l$ with standard terms for collision avoidance, lane keeping, goal reaching, and ride comfort; and a dynamically extended unicycle model~\cite{lavalle2006better} for the vehicle dynamics.

Next we provide a formal discussion of the \algname{} algorithm.
% \section{Contingency planner}\label{sec:DP}
% The contingency planner takes the ego trajectory tree $\bfr$ and the scenario tree $\bfe$ generated by the prediction module (which could be ego-conditioned or not) and generates a closed-loop policy with dynamic programming. 

% Intuitively, with the scenario tree and trajectory tree constructed, the continuous planning problem reduces to a discrete MDP. States of the MDP are branches of the scenario/trajectory trees that represent the joint ego and environment state; transitions are given by the tree parent/children edges in the two trees. We then solve for the optimal finite-horizon \emph{policy} for the discrete MDP using dynamic programming, i.e., calculating the value function backwards in stage via the Bellman equation. With the optimal policy, the continuous-time trajectory is recovered from the trajectory tree by executing the trajectory segments according to the policy.

\section{Formal discussion}\label{sec:formal}

\subsection{Analysis without ego-conditioning}
In our motion planning problem we are interested in minimizing the expected cumulative cost over a horizon:
\begin{equation*}
    \mathcal{J} = \int_{0}^T l(s(t),s_e(t))dt,
\end{equation*}
where $l$ is the running cost function that depends on the ego state $s$ and the environment state $s_e$, $T$ is the planning horizon.  Our planning algorithm operates on the two trees $\bfr$ and $\bfe$ with the same number of stages, so the cumulative cost can be rewritten as 
\begin{equation}\label{eq:stage_cumu_cost}
    \mathcal{J} = \sum_{i=0}^{N} L_i(r^i,e^i),
\end{equation}
where $r^i$ and $e^i$ are the nodes the ego vehicle and the environment take at stage $i$, and $L_i(r^i,e^i)=\int_{t^i_0}^{t^i_f} l(s^{r^i}(t),s_e^{e^i}(t)) dt$. Due to the stochasticity of the environment, we aim to minimize $\mathbb{E}_{e^{0:N}}[\sum_{i=0}^{N} L_i(r^i,e^i)]$, where the expectation is on $e^i$, the actual branch the environment takes and the distribution is given as part of the prediction. For simplicity, we shall present the result assuming $\bfe$ is not ego-conditioned, i.e., there is a single $\bfe$, and later show that the result can be easily extended to the case with ego-conditioning.

The end result is a policy that chooses which node to execute for the next stage given the current ego and environment node, i.e., $r^{i+1} = \pi^\star(r^i,e^i)$, where $\pi^\star$ is the optimal policy. The form of the policy is determined by the assumption about the information flow, i.e., during stage $i$, the ego vehicle can observe the environment's response $e^i$, and choose the ego motion among the children nodes of the current node $r^i$. To obtain the optimal policy, a value function is needed:
\begin{equation}\label{eq:V}
    V(r^i,e^i)=\mathbb{E}_{e^{i:N}} [\sum_{k=i}^N L_k(r^k,e^k)],
\end{equation}
which is the expected cost-to-go. The dynamic program goes backwards in stage and is trivial for the last stage:
\begin{equation*}
    V(r^N,e^N)=L_N(r^N,e^N).
\end{equation*}
For stage i where $i<N$, we have
\begin{equation*}
    V(r^i,e^i) = L_i(r^i,e^i)+\min_{r^{i+1}\in \ch(r^i)}\mathbb{E}_{e^{i+1}}[V(r^{i+1},e^{i+1})|e^i].
\end{equation*}
Since $e^{i+1}$ is enumerable, the expectation is calculated as 
\begin{equation*}
    \mathbb{E}_{e^{i+1}}[V(r^{i+1},e^{i+1})|e^i] = \sum_{e^{i+1}_j\in\ch(e^i)} \mathbb{P}[e^{i+1}_j|e^i] V(r^{i+1},e^{i+1}_j),
\end{equation*}
where the branching probability of the scenario tree is given by the prediction model. Further define
\begin{equation*}
\begin{aligned}
    Q(r^{i+1},e^i)&:=L_i(r^i,e^i)+\mathbb{E}_{e^{i+1}}[V(r^{i+1},e^{i+1})|e^i]\\ &= L_i(r^i,e^i)+\sum_{e^{i+1}_j\in\ch(e^i)} \mathbb{P}[e^{i+1}_j|e^i] V(r^{i+1},e^{i+1}_j).
    \end{aligned}
\end{equation*}
where $r^i=\pa(r^{i+1})$.
We name this function $Q$ function as it is analogous to the $Q$ function in reinforcement learning where here $b^{k+1}$ is the action we need to choose.

The value function is then obtained backwards in stage:
\begin{equation}
    V(r^i,e^i)=\left\{\begin{array}{cc}L_i(r^i,e^i),&i=N\\\min_{r^{i+1}\in \ch(r^i)}Q(r^{i+1},e^i),&i<N \end{array}\right.
\end{equation}
The optimal policy is then
\begin{equation}\label{eq:opt_policy}
    \pi^\star(r^i,e^i)=\mathop{\arg\min}_{r^{i+1}\in\ch(r^i)} Q(r^{i+1},e^i).
\end{equation}

\noindent\begin{thm}[Optimality]\label{thm:DP}
The policy in \eqref{eq:opt_policy} is the optimal policy with respect to the cost in \eqref{eq:stage_cumu_cost}.
\end{thm}
\noindent\begin{proof}
The proof is by induction. For stage $N$, the cost is a constant, $\pi^\star$ is trivially optimal, and $V(r^N,e^N)$ is the cost-to-go. For $0\le i<N$, assume $V(r^{i+1},e^{i+1})$ is the expected cost-to-go function at stage $i+1$, then by the principle of optimality, the optimal node to take at stage $i+1$ is
\begin{equation*}
    r^{i+1,\star}=\mathop{\arg\min}_{r^{i+1}\in\ch(r^i)} L_i(r^i,e^i)+\mathbb{E}_{e^{i+1}}[V(r^{i+1},e^{i+1})|e^i],
\end{equation*}
which is exactly $\pi^\star(r^i,e^i)$. This in turn shows that 
\begin{equation*}
\begin{aligned}
    V(r^i,e^i) &= L_i(r^i,e^i)+\mathbb{E}_{e^{i+1}}[V(r^{i+1,\star},e^{i+1})|e^i]\\
    &=\min_{r^{i+1}\in \ch(r^i)}Q(r^{i+1},e^i).
\end{aligned}
\end{equation*}
This is true for all nodes in $\bfr$ and $\bfe$, then by induction, $\pi^\star(s^i,e^i)$ is the optimal policy for all $i\in\{0,1,...,N\}$.
\end{proof}

\subsection{Extension to ego-conditioned prediction.}
% \noindent \textbf{Extension to ego-conditioned prediction.}
In the case where the scenario tree is ego-conditioned, the algorithm structure stays roughly the same. To generate the ego-conditioned trajectory prediction, we first run the ego motion sampler to generate the trajectory tree, then the trajectory tree is "flattened " to create the ego-conditioning (EC) modes. E.g., for trees in Fig. \ref{fig:diagram}, the flattened EC modes are shown in Fig. \ref{fig:EC}.
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{batch_from_tree.png}
    \caption{Flattened trajectory tree as ego-conditioning modes}
    \label{fig:EC}
    \vspace{-0.6cm}
\end{figure}
Under each EC mode, the prediction model generates a distinct scenario tree conditioned on the ego vehicle's motion. To keep the planning problem under ego-conditioning well-defined, the ensemble of EC scenario trees needs to satisfy a condition called causal consistency. 
\begin{definition}[Causal consistency]\label{def:consistency}
The ensemble of EC scenario tree is causally consistent (CC) if for any stage $i\le N$, any two scenario trees under different EC modes, if the conditioned ego trajectories are identical up to stage $i$, the two scenario trees are identical up to stage $i$.
\end{definition}

This condition guarantees the causality of the policy planning problem as for any particular stage $i$ within the prediction horizon, no future information beyond stage $i$ affects the prediction up to stage $i$. While causal consistency seems trivial, it may be violated by a multi-stage prediction model without special care. For example, if the EC trajectory is encoded as a whole for all stages, the scenario trees generated are not causally consistent.
\begin{prop}[Sufficient condition for CC]
Assume that a multi-stage ego-conditioned prediction model generates the trajectory prediction stage by stage and the EC prediction is deterministic, then the generated ensemble of EC scenario trees is causally consistent.
\end{prop}
\begin{remark}
For stochastic prediction models, the generated scenario trees are causally consistent if the random seeds are shared among all EC modes with the same EC trajectory.
\end{remark}

The proof is omitted here. It is straightforward to show that the 3 prediction models in Section \ref{sec:pred} are CC. 


Given causally consistent EC predictions, only two terms change in the policy planning algorithm. First, all nodes of the scenario tree now depend on one of the nodes of trajectory tree of the same stage, and are denoted as $e^i(r^i)$ to emphasize the dependence. Note that the dependence is on $r^i$ instead of the whole ego trajectory due to causal consistency. Second, the branching probability now depends on the ego node, and is denoted as $\mathbb{P}[e^{i+1}_j|e^i(r^i),r^i]$.

Formally, we are solving a finite-horizon MDP with a joint state of $(r^i,e^i)$ and the cost defined in \eqref{eq:stage_cumu_cost}. The action space is $A(r^i)=\ch{r^i}$, the next ego maneuver, and the transition probability is 
\begin{equation*}
\resizebox{1\columnwidth}{!}{$
    \mathbb{P}[(r^{i+1},e^{i+1})|(r^i,e^i(r^i)),r^{i+1}_j] = 
    \left\{ \begin{aligned}
        &\mathbb{P}[e^{i+1}(r^{i+1}_j)|e^i(r^i),r^i],& \textbf{if}\; r^{i+1}=r^{i+1}_j\\
        &0,& \textbf{otherwise}
    \end{aligned} \right.
    $}
\end{equation*}
Interestingly, the value function can be defined exactly the same way as
\begin{equation}\label{eq:EC_V}
    V(r^i,e^i(r^i))=\mathbb{E}_{e^{i:N}} [\sum_{k=i}^N L_k(r^k,e^k(r^k))].
\end{equation}
Similarly, the Q function is now
\begin{equation*}
\resizebox{1\columnwidth}{!}{$
\begin{aligned}
    Q(r^{i+1},e^i(r^i))&:=L_i(r^i,e^i(r^i))+\mathbb{E}_{e^{i+1}}[V(r^{i+1},e^{i+1}(r^{i+1}))|e^i(r^i)]\\ &= L_i(r^i,e^i(r^i))+\sum_{e^{i+1}_j\in\ch(e^i(r^{i}),r^{i+1})} \mathbb{P}[e^{i+1}_j|e^i(r^i),r^i] V(r^{i+1},e^{i+1}_j),
    \end{aligned}
$}
\end{equation*}
where $\ch(e^i(r^{i}),r^{i+1})$ denotes the set of children nodes following $e^i(r^{i})$ on the tree associated with $r^{i+1}$.
The optimal policy is then defined as
\begin{equation}\label{eq:EC_opt_policy}
    \pi^\star(r^i,e^i(r^i))=\mathop{\arg\min}_{r^{i+1}\in\ch(r^i)} Q(r^{i+1},e^i(r^i)).
\end{equation}

\noindent\begin{thm}
Given a causally consistent ensemble of EC scenario trees, the policy in \eqref{eq:EC_opt_policy} is the optimal policy with respect to the cost function $\mathcal{J} = \sum_{i=0}^{N} L_i(r^i,e^i(r^i)).$
\end{thm}

\noindent\begin{proof}
The proof essentially follows the same steps as the proof of Theorem \ref{thm:DP}. Starting from stage $N$, the cost is constant, thus $\pi^\star$ is trivially optimal and $V(r^N,e^N(r^N))$ is the cost-to-go. For all $0\le i <N$, assume for all $r^{i+1}$, $V(r^{i+1},e^{i+1}(r^{i+1}))$ is the expected cost-to-go function at stage $i+1$. Then for any $r^i$, the cost-to-go to take any children node $r^{i+1}\in\ch(r^i)$ is $L_i(r^i,e^i(r^i))+\mathbb{E}[V(r^{i+1},e^{i+1}(r^{i+1}))|e^i(r^i)]$,
which is exactly $Q(r^{i+1},e^i(r^i))$. It follows that $\pi^\star(r^i,e^i(r^i))$ gives the optimal $b^{i+1}$ within $\ch(r^i)$ and the cost-to-go function of stage $i$ is computed as
\begin{equation*}
    V(r^i,e^i(r^i)) = \min_{r^{i+1}\in \ch(r^i)}Q(r^{i+1},e^i(r^i)).
\end{equation*}
The optimality of $\pi^\star$ is then proved by induction.
\end{proof}



==> [Chen.ea.ICRA.22]Contingency planning/experiment.tex <==

\section{Experiments}\label{sec:experiment}

\begin{table}[]
\begin{tabular}{c|ccc}
                 & Rasterized & PredictionNet & Agentformer \\ \hline
Mean ADE      & 0.67       & 0.25          & 0.33        \\
Mean FDE      & 1.3        & 0.85          & 1.01        \\
\end{tabular}
\caption{Prediction metrics average displacement error (ADE) and final displacement error (FDE) of the three models. The mean is taken over all modes.}
\label{tab:prediction}
\vspace{-0.5cm}
\end{table}

\subsection{Training of prediction model}
We configure \algname{} with three different prediction models. Apart from the model architecture, the experimental setup is the same. Prediction models are trained with the nuScenes dataset \cite{caesar2020nuscenes}, comprised of 1000 scenes lasting for 20 seconds collected in urban areas of Boston and Singapore. For simplicity, only vehicles are considered. All prediction models use 2 stages and the branching factor is 4. % While the model structures are different, they share a few common setups.

% \noindent\textbf{Cost function.} Besides some model-specific terms, the common cost terms consist of 
\textbf{Loss function.} Our training loss is a weighted sum of the following terms: prediction loss that penalizes the error between the predicted trajectories and the ground truth; EC collision loss that penalizes collisions between the predicted trajectories and the conditioned ego trajectory;  collision loss that penalizes collisions between predicted trajectories of different agents in the scene; and additional standard regularization losses specific to the model architecture. 
% regularization loss, penalizes the 2-norm of predicted input signals when dynamic model is used to generate the trajectory prediction.
% \begin{itemize}
    % \item prediction loss, penalizes the error between the predicted trajectory and the ground truth;
    % \item EC collision loss, penalizes collisions between the predicted trajectories and the conditioned ego trajectory;
    % \item collision loss, penalizes collisions between predicted trajectories of different agents in the scene;
    % \item input regularization loss, penalizes the 2-norm of predicted input signals when dynamic model is used to generate the trajectory prediction.
% \end{itemize}

% \noindent\textbf{Dynamic model.} We use the same unicycle model as in \eqref{eq:unicycle} with Euler discretization as the dynamic model for vehicles. Kinematic and dynamic constraints such as friction limits and minimum turning radius are also added to guarantee the dynamic feasibility of the generated trajectories.

\myparagraph{Ego conditioning.} One natural choice of the ego trajectory for ego-conditioning is the ground truth future trajectory. In addition, to expose the model to more diverse ego trajectories, we perturb the ground truth ego trajectory with noise generated via the \textit{Ornstein–Uhlenbeck} process as alternative ego trajectories. However, since the ground truth for surrounding agents under the counterfactual ego motion is not available, for the lack of a better choice, we still use the original ground truth as the target for the EC trajectory prediction. We penalize collision between the predicted trajectories of surrounding agents and the conditioned ego trajectory so that the model learns to avoid the conditioned ego trajectory.

\myparagraph{Training results.} We report standard ADE/FDE prediction metrics for the three prediction models in Table \ref{tab:prediction}. The results show that all three models learn reasonable predictions.


\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{contingency_sim.png}
    \caption{Example scene from simulation: the ego vehicle (blue) cuts in front of the red vehicle and then swerve around the green static vehicle in front. The ego trajectory tree is shown in magenta, the colored line shows agents' actual trajectory.}
    \label{fig:sim_snapshot}
    \vspace{-0.5cm}
\end{figure}

% \subsection{Closed-loop simulation}\label{sec:sim}
\subsection{Experimental setup}\label{sec:setup}

\myparagraph{Closed-loop simulation.} We evaluate \algname{} in BITS, a closed-loop AV simulation environment proposed in \cite{BITS}. Each simulation scene is initialized with a scene from the nuScenes dataset and then evolves forward with a policy for each agent. One agent is chosen as the ego vehicle and controlled by \algname{} or its alternatives. All other agents runs the learned BITS policy that generates realistic and diverse behavior of road vehicles. Additionally, to incite more interactions between agents, we "spawn" new agents around the ego vehicle to challenge the planner throughout the simulation duration.
% This is because in traffic simulation stochasticity and agents' effort to avoid collision lead to agents moving away from each other as time goes on. 

\myparagraph{Metrics.} We use three key metrics: collision rate, offroad rate, and area coverage. The first two are calculated as the percentage of time steps where the ego vehicle is in collision (offroad). The coverage metric is calculated with a kernel density estimation (KDE) procedure following~\cite{BITS}, and it captures the effectiveness of the ego plan in terms of liveness and distance travelled.  %In particular, we use a grid of the map and count the grid points that are passed by the ego vehicle as a measure of liveness. 
The evaluation is done on 100 scenes from the evaluation split of nuScenes (not used for training).

\myparagraph{Baselines.} We consider three baselines, the first two are non-contingent counterpart of \algname{}. For fair comparison, the two baselines share the same ego-motion sampler and ego-conditioning prediction model as \algname{}, the first baseline, named non-contingency robust (NCR), considers all possible trajectories predicted by the prediction model (similar to \cite{chen2020reactive}); while the second baseline, named non-policy greedy (NCG), only avoids the most likely prediction mode (similar to \cite{xu2014motion}). The third baseline uses a kinematic prediction model with 2 modes: maintaining speed and braking, and share the same multi-stage tree structure. 



\bgroup
\setlength{\tabcolsep}{2pt}
\begin{table}[]
\vspace{-0.3cm}
\centering
\begin{tabular}{l|c|ccc}
  % & Pred. model  & Crash rate  & Offroad rate & Coverage \\ 
 Planning  & Prediction   & Crash         & Offroad      & Coverage $\uparrow$\\ 
 algorithm & model       & rate $\downarrow$  & rate $\downarrow$ &   \\ 
\hline
TPP (ours) & Rasterized  & \textbf{0.46\%}     & \textbf{0.64\%}       & 164      \\
Non-Cont. Robust & Rasterized  & 0.80\%     & 0.61\%       & 163      \\
Non-Cont. Greedy & Rasterized  & 1.23\%     & 1.00\%       & \textbf{168}      \\
\hline
TPP (ours) & PredictionNet  & \textbf{1.02\%}     & \textbf{0.10\%}       &\textbf{174}      \\
Non-Cont. Robust & PredictionNet  & 1.34\%     & 2.07\%       & 166      \\
Non-Cont. Greedy & PredictionNet  & 1.60\%     & 0.45\%       & 170      \\
\hline
TPP (ours) & Agentformer  & \textbf{0.97\%}     & \textbf{0.20\%}       & \textbf{174}      \\
Non-Cont. Robust & Agentformer  & 1.08\%     & 0.63\%       & 158      \\
Non-Cont. Greedy & Agentformer  & 2.52\%     & 0.98\%       & 163      \\
\hline
TPP (ours) & Agentformer (Gaussian)  & 3.92\%     & 5.53\%       & 150      \\
Non-Cont. Robust & Agentformer (Gaussian)  & 1.40\%     & 0.40\%       & 144      \\
Non-Cont. Greedy & Agentformer (Gaussian) & 1.04\%     & 0.25\%       & 149      \\
\hline
TPP (ours) & Kinematic model & 1.75\% & 0.51\%  &160\\
\end{tabular}
\caption{Closed loop simulation results with \algname{} and the baselines, the default Agentformer model uses a discrete latent space and Agentformer (Gaussian) is its variant with a Gaussian latent space. \algname{} significantly outperform the baselines with the same ego trajectory tree and prediction model (bold means best).}
\label{table:metrics}
\vspace{-0.5cm}
\end{table}
\egroup
% \bgroup
% \setlength{\tabcolsep}{0.2pt}
% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc}
%              & TPP                     & NCR              & NCG             \\ \hline
% Crash rate   & \textbf{(0.46\%, 1.0\%, 0.97\%)} & (0.8\%, 1.3\%, 1.1\%) & (1.2\%, 1.6\%, 2.5\%)  \\
% Offroad rate & \textbf{(0.6\%, 0.1\%, 0.2\%)}   & (0.61\%, 2.1\%, 0.6\%)  & (1.0\%, 0.45\%, 1.0\%) \\
% Coverage     & (164, \textbf{174, 174})          & (163, 166, 158)        & (\textbf{168}, 170, 163)    
% \end{tabular}
% \caption{Metrics of the closed loop simulation. The 3 numbers correspond to the simulation under the rasterized model, PredictionNet, and Agentformer, and their average. Our \algname{} significantly outperform the benchmarks with the same ego trajectory tree and prediction model. }
% \label{table:metrics}
% \vspace{-0.5cm}
% \end{table}
% \egroup

\subsection{Results}\label{sec:result}
Fig. \ref{fig:sim_snapshot}  shows snapshots of the simulation with \algname{} where the ego vehicle (blue) cuts in front of the red vehicle and then change lane again to avoid the parked green vehicle. The magenta lines show the ego trajectory tree, and the colorful line shows the rollout trajectories of the agents. The quantitative results are shown in Tables \ref{table:metrics} and \ref{table:EC}, and we make the following observations. Simulation videos can be found \href{https://sites.google.com/nvidia.com/avg-tpp/home}{here}.

\myparagraph{TPP outperforms the baselines.}
As shown in Table \ref{table:metrics}, \algname{} significantly outperforms the two non-policy baselines on crash and offroad rate under all 3 prediction models while achieving similar coverage. Even under a simple kinematic model, the performance is better than non-policy planners with sophisticated prediction models. \algname{} with deep-learned prediction models performs better than with a simple kinematic model, indicating the deep-learned prediction model benefits the closed-loop performance. 



\myparagraph{Better predictions do not mean better plan.}
Interestingly, from Table \ref{table:metrics}, the "better" prediction model measured by ADE/FDE does not necessarily lead to better closed-loop performance. For example, the rasterized model is the simplest and "worst" model among the three, yet \algname{} with it outperforms the other two in terms of crash rate.

\myparagraph{Ego-conditioning is useful.} Table \ref{table:EC} compares \algname{} with or without ego-conditioning. Ego-conditioning improves the closed-loop performance considerably in most cases, especially the coverage metric, hinting that the ego vehicle is more comfortable moving through traffic when it expects reaction from other agents.

\myparagraph{Temporal consistency is important.} Additionally, we tested the Agentformer model with Gaussian latent space, where the prediction requires sampling of the latent variable at every inference call, compared to using discrete latent space where sampling is not needed. While the prediction ADE/FDE is similar, the closed-loop performance with the Gaussian latent is significantly worse. % (results are excluded from Table \ref{table:metrics}). 
We suspect this is due to the poor temporal consistency between predictions of consecutive time steps. While both \algname{} and the two baselines saw performance degradation under the Gaussian latent, the policy planner relies on more sophisticated prediction/planning interaction, thus suffers more than the two baselines.










\begin{table}[]
\centering
\begin{tabular}{c|ccc}
                   & Crash rate$\downarrow$ & Offroad rate$\downarrow$ & Coverage $\uparrow$\\ \hline
Rasterized   & \textbf{0.46\%} / 0.53\%     & \textbf{0.60\%} / 1.05\%       & \textbf{164} / 163     \\
PredictionNet   & 1.00\% / \textbf{0.63\% }   & \textbf{0.10\%} / 0.71\%     & \textbf{174} / 151     \\
Agentformer  & \textbf{0.97\%} / 1.30\%    & \textbf{0.20\%} / 0.53\%      & \textbf{174} / 163     \\
\end{tabular}
\caption{\comment{this can be easily merged with Table III to save space } Ablation study of ego-conditioning, the first and second number are the metrics with and without ego conditioning. Most metrics see degradation when ego-conditioning is disabled (bold means better).}
\label{table:EC}
\vspace{-0.4cm}
\end{table}

% We make the following observations.


% 1. \algname{} significantly outperforms the two non-contingent baselines on crash rate and offroad rate under all 3 prediction models while achieving similar coverage. Even under a simple kinematic model, the performance is better than non-contingent planners with sophisticated prediction models.

% 2. \algname{} under deep-learned prediction models outperforms itself under a simple kinematic model, indicating the deep-learned prediction benefits the closed-loop performance. However, the "better" prediction model measured by ADE/FDE does not necessarily lead to better closed-loop performance. For example, the rasterized model is the simplest and "worst" model among the three, yet \algname{} outperforms the other two models in terms of crash rate.

% 3. Temporal consistency is very important to closed-loop performance. We tested the agentformer model with Gaussian latent space, where the prediction requires sampling of the latent variable, and discrete latent space where sampling is not needed. While the ADE/FDE is similar, the closed-loop performance with the Gaussian kernel is significantly worse. We suspect this is due to the poor temporal consistency between predictions of consecutive time steps. While both \algname{} and the two baselines saw performance degradation under the Gaussian latent, the contingency planner relies on more sophisticated prediction of the future, thus suffers more than the two baselines.

% 4. Ego-conditioning improves the closed-loop performance of \algname{} considerably in most cases, especially the coverage metric, hinting that the ego is more comfortable moving through traffic when it expects reaction from other agents.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{l|ccc}
                    & Rasterized & PredictionNet & Agentformer \\ \hline
Prediction w/ EC    & 150ms      &   5.00s            &    2.60s        \\
Prediction w/o EC   &  37ms       & 75ms          & 150ms       \\
Ego-motion sampling & & 30ms &              \\
Dynamic programming & & 11ms &                
\end{tabular}
\caption{Runtime of the three key components}
\label{table:runtime}
\vspace{-0.5cm}
\end{table}

\myparagraph{Runtime analysis.}
Table \ref{table:runtime} shows the runtime of the three components of \algname{} on an Nvidia 3090 GPU (most computation is done on GPU). It should be noted that all runtime is recorded on unoptimized Python code and there is significant space of improvement. For example, the long runtime for PredictionNet is mainly due to rasterization, and we know its runtime can be as low as 5ms with the proper engineering \cite{predictionnet}, e.g., efficient CUDA code for rasterization. 
 %Another reason for the long runtime of prediction is due to limited GPU memory. Since with ego-condtioning, we are generating $M^N$ scenario trees simultaneously, where $M$ is the branching factor and $N$ is the number of stages, we quicky run out of GPU memory and need to run in smaller batches sequentially.
 While the runtime for prediction models is not very informative and is not the focus of this paper, it is quite clear that ego motion sampling and dynamic programming can be done very efficiently. With proper optimization, we believe that \algname{} can be easily implemented in real time. We plan to release the code upon publication.


==> [Chen.ea.ICRA.22]Contingency planning/introduction.tex <==
% \section{INTRODUCTION}\label{sec:intro}
% One key challenge of motion planning for autonomous vehicles is handling the interactions with nearby agents, which involves two subproblems, trajectory prediction and motion planning with prediction. The task of trajectory prediction has been studied extensively, ranging from kinematic models \cite{kong2015kinematic}, maneuver recognition \cite{houenou2013vehicle}, to the various deep learning models that pushed the state-of-the-art in recent years \cite{predictionnet,T++,rhinehart2019precog,ILVM,ScePT}. These models typically generate multimodal predictions and are trained to 
% % minimize the mean prediction error given a dataset of driving logs. 
% % On the other hand, a typical planner leverages the prediction result by considering a single trajectory prediction \cite{xu2014motion}, multiple trajectory predictions \cite{cui2021lookout}, and occupancy prediction \cite{plan_occu,sadat2020perceive}. 
% maximize the likelihood of a dataset of driving logs under the model.
% A typical planner then uses the prediction result either by considering a single trajectory prediction~\cite{xu2014motion}, multiple trajectory predictions~\cite{cui2021lookout}, or occupancy predictions~\cite{plan_occu,sadat2020perceive}. 

% % One key drawback with traditional trajectory planning is that the planned trajectory is expected to perform well under all predicted modes of the scene evolution, while in reality, human drivers usually react to the scene evolution rather than committing to a single trajectory. Although the scene evolution beyond the current time is unknown, we can take advantage of the prediction model to enumerate possible scene evolution modes and condition the ego motion plan on the future scene evolution. This is exactly the motivation for contingency planning, which generates a motion policy instead of a single trajectory in preparation for the different possible environment behavior. 
% An important drawback of traditional trajectory planning is that it seeks a single trajectory that performs well under \emph{all} predicted modes of the scene evolution, ignoring the fact that 1) some modes of the future are mutually exclusive and 2) the AV will be able to replan with more information in a future time step. Contingency planning addresses this problem: it generates a \emph{motion policy} instead of a single trajectory, taking advantage of the prediction model to enumerate possible scene evolution modes and conditioning the ego motion plan on the future scene evolution. The main difference between a motion policy and a single trajectory is that a motion policy conditions the trajectory to execute on future observations of the environment.



% \begin{ex}\label{ex:motivating}
% Consider a task of passing by a vehicle on the adjacent lane depicted on the right end in Fig. \ref{fig:diagram}. Within the planning horizon, the adjacent vehicle may maintain its current lane or cut in front of the ego vehicle. A non-contingency motion plan seeks a single trajectory that performs well in both situations and thus will not choose to complete the pass due to the risk of collision should the adjacent vehicle choose to change lane. A contingency motion plan may choose to move forward for 1 second, observe the behavior of the adjacent vehicle, and then decide the subsequent motion. If the adjacent vehicle has no intention of lane change, the ego vehicle proceeds with the passing, otherwise slows down. 
% \end{ex}




% % \begin{figure}
% %     \centering
% %     \includegraphics[width=1\columnwidth]{contingency_hero.png}
% %     \caption{Contingency planning in the case of example \ref{ex:motivating}: the ego vehicle (blue) prepares a trajectory tree with multiple branches at each stage; the future motion of the human-driven vehicle (red) is predicted in the form of a scenario tree, and the contingency planner generates a policy that decides the branch to execute from the trajectory tree based on future observations of the human-driven vehicle (closest branch in the scenario tree). The actual chosen trajectory is solid whereas the unrealized branches are transparent.}
% %     \label{fig:example}
% %     \vspace{-0.5cm}
% % \end{figure}

% The early works on contingency planning date back to the Darpa challenge, where \cite{hardy2013contingency} proposed a trajectory optimization method with one trajectory for each scene evolution mode, which are enumerated with a predefined set of possible actions for the dynamic obstacles. Similar ideas are also seen in \cite{zhan2016non,galceran2017multipolicy} where a predefined set of modes are evaluated online. In \cite{chen2022interactive}, the trajectory optimization is solved with a branch Model Predictive Control (MPC) algorithm that enables mutli-stage planning and allow the scene evolution to be dependent on the ego motion (ego-conditioning). Due to the nature of gradient-based optimization, the environment model needs to be differentiable if ego-conditioning is used, which limits the model complexity. \cite{cui2021lookout} uses an MPC with a deep-learned prediction model, yet does not use ego-conditioning. Apart from the optimization-based approaches, sampling-based planning is also extended to contingency planning, one prominent example is Partially Observed Markov Decision Process (POMDP) \cite{bai2015intention,liu2015situation,intentionaware}, where the action space is discretized and the future actions depend on future observations of the environment. The game theoretic approach sits on the borderline between contingency planning and traditional motion planning as it leverages the reaction from the environment, yet assumes some fixed behavior model of the environment, e.g. rational \cite{sadigh2016planning} or noisy Boltzmann policy \cite{fisac2019hierarchical}, which tends to be uni-modal. In \cite{rhinehart2021contingencies}, contingency planning takes the form of a neural network trained to react to the environment behavior and ego latent, which can incorporate sophisticated environment models but is not interpretable.

% \textit{Desiderata} To meet the requirements of practical autonomous driving, we seek a contingency planning algorithm with the following desired features (1) compatible with state-of-the-art deep-learned predictive models (2) capable of ego-conditioning, i.e., factor in ego vehicle's influence on nearby agents (3) interpretable and easily tunable (4) allow for multistage reasoning that leverages agents' future reactive behavior (5) scale to scenarios with a large number of agents.

% To achieve the desiderata, \algname{} takes a sampling-based approach and consists of three key components: an ego motion sampler that generates ego trajectory trees, a deep-learned multi-stage prediction model that generates scenario trees, and a contingency planner that solves for the optimal finite-horizon policy for the ego vehicle. Table \ref{table:exist_method} summarizes some existing contingency planning methods found in literature together with \algname{} and we would like to show that \algname{} can fill the gap to our desiderata.

% \comment{would be good to summarize experiments and results at the end of intro}




%%%%%%%%%%%%%%%%

\section{Introduction}\label{sec:intro}

%% problem setup 
A key challenge of motion planning for autonomous vehicles (AV)s is reasoning about the interaction between the ego vehicle and  neighboring agents. %, e.g., vehicles, cyclists, pedestrians. 
The task is commonly divided into two subproblems: trajectory prediction for other agents, and ego motion planning with prediction. 
Trajectory prediction has seen substantial progress in recent years, coming from simple kineamtic models \cite{kong2015kinematic} to powerful deep learning models \cite{predictionnet,T++,rhinehart2019precog,ILVM,ScePT} capable of generating high-quality, multi-modal predictions. However, motion planning with such high-capacity prediction models remains a challenge.

% challenge of planning
Typical AV planners simplify the ego behavior planning problem into \emph{trajectory planning}, where a single trajectory is sought that minimizes an expected cost over \emph{all} predicted futures within the planning horizon~\cite{xu2014motion}. 
Such trajectory planning leads to overly conservative plans because it ignores the new information to be acquired about other agents in subsequent time steps, and the effects of ego actions on the behavior of other agents.

In fact, in decision-making literature, people have long been pursuing a closed-loop policy instead of an open-loop plan as the former is shown to be optimal for problems such as Markov decision processes (MDP) \cite{puterman1990markov}. 

\bgroup
\setlength{\tabcolsep}{4pt}
\begin{table}[b]
\vspace{-0.4cm}
\begin{tabular}{l|ccccc}& DL & EC  & Interp & MS & Scalability \\\hline
Multi-mode planning
\cite{hardy2010contingency, hardy2013contingency,zhan2016non,galceran2017multipolicy} &  $\xm$  &  $\xm$  & $\ck$ &$\xm$ & poor \\
Branch MPC \cite{chen2022interactive} & $\xm$  & $\ck$ & $\ck$&  $\ck$ & poor\\
POMDP \cite{bai2015intention,liu2015situation,intentionaware}  & $\xm$ &  $\ck$  &$\ck$ &$\ck$ & poor\\

Game theoretic \cite{fisac2019hierarchical,sadigh2016planning}  & $\xm$   &   $\ck$  & $\ck$ &$\xm$  & very poor     \\
Lookout \cite{cui2021lookout}    &   $\ck$ &  $\xm$   &      $\ck$  &$\xm$    & good   \\
CfO \cite{CfO}   &$\ck$  & $\ck$ &  $\xm$ & $\xm$ & medium \\
\algname{} (ours)  & $\ck$ &  $\ck$  &   $\ck$ & $\ck$ & good
\end{tabular}
\caption{Comparison of existing policy planning methods and \algname{} where ``DL'' is short for compatibility with deep-learned prediction models, ``EC'' stands for ego-conditioning, ``Interp'' is short for interpretable, ``MS'' stands for multistage, and ``Scalability'' means the capability to scale to complicated scenes with large number of agents.}
\label{table:exist_method}
\vspace{-0.5cm}
\end{table}

\egroup


\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{diagram.png}
    \caption{Structure of \algname{}: the ego motion sampler generates the trajectory tree, which is fed to the prediction model for ego-conditioned prediction to generate the scenario tree. Then we solve for the ego motion policy via dynamic programming.}
    \label{fig:diagram}
    \vspace{-0.6cm}
\end{figure*}
% A typical planner then uses the prediction result either by considering a single trajectory prediction~\cite{xu2014motion}, multiple trajectory predictions~\cite{cui2021lookout}, or occupancy prediction~\cite{plan_occu,sadat2020perceive}. 
% An important drawback of traditional trajectory planning is that it seeks a single trajectory that performs well under \emph{all} predicted modes of the scene evolution, ignoring the fact that 1) some modes of the future are mutually exclusive and 2) the AV will be able to replan with more information in a future time step. Contingency planning addresses this problem: instead of a single trajectory it generates a \emph{motion policy}  

% illustrative example
To highlight the difference between a \emph{motion policy} and a single trajectory, consider the scenario depicted on the right end of Fig. \ref{fig:diagram}. The ego vehicle (blue) needs to move pass the adjacent vehicle (red). Within the planning horizon, the red vehicle either maintains its current lane or cuts in front of the ego vehicle. A traditional planner seeks a single trajectory that performs well in both situations and thus will not choose to pass since lane change is a plausible choice for the red vehicle at current time. Alternatively, a motion policy may choose to nudge forward for the first part of the horizon, observe (by leveraging a forecasting model) the behavior of the adjacent vehicle, and then decide the subsequent motion. If the red vehicle already started a lane change, the ego vehicle brakes to avoid collision; if the red vehicle stays in its own lane, since the ego vehicle is already next to the red vehicle, a sudden lane change is very unlikely, the ego vehicle can then move past the red vehicle. 

In the field of robotics, policy planning often takes the form of \emph{contingency planning}~\cite{hardy2013contingency,zhan2016non}, with the key idea of preparing multiple plans for different likely futures. To differentiate the two concepts, we view contingency planning as a simplified policy planning variant with only one stage of reasoning. Unfortunately, continuous-space policy planning with high-capacity prediction models is computationally prohibitive, and despite various simplifications ~\cite{chen2022interactive,cui2021lookout,bai2015intention}, practical policy planning for AVs remains an open problem.

% what we want in this paper
In this paper we introduce Tree Policy Planning (\algname{}), a practical policy planner that meets the requirements of real-world autonomous driving, specifically, \algname{} is designed with the following desiderata:
\begin{enumerate}
    \item compatible with state-of-the-art deep-learned predictive models for trajectory forecasting 
    \item plans with closed-loop ego-conditioning, i.e., factors in the ego vehicle's influence on other agents
    \item allows for multistage reasoning that leverages the agents' future reactive behavior
    \item interpretable and easily tunable 
    \item scales to scenarios with a large number of agents
\end{enumerate}
We compare existing policy planning works with TPP in Table \ref{table:exist_method}. To the best of our knowledge, TPP is the first algorithm that fulfils our desiderata.

% details of our approach
The key idea of \algname{} is to convert the continuous space motion planning problem into a tractable finite-horizon MDP by constructing two trees: an \emph{ego trajectory tree} carrying ego motion candidates, and a \emph{scenario tree} that contains multiple behavior modes for neighboring agents. The algorithm is illustrated in Fig.~\ref{fig:diagram}. It consists of three components: an ego motion sampler that generates the ego trajectory tree, a deep-learned multi-stage prediction model that generates the scenario tree, and a dynamic program module that solves for the optimal policy with respect to the constructed MDP. 
% In this manner, TPP can generate multi-stage contingency plans with powerful prediction models in the loop that account for the influence of the ego vehicle on others. 
%  \comment{maybe say sth about our formal results.} 

% results
We evaluate \algname{} in closed-loop simulation based on a recently proposed realistic data-driven traffic model~\cite{BITS}. Our results show that \algname{} achieves good closed-loop driving performance in real-world scenarios from the nuScenes dataset \cite{nuscenes}, and significantly outperforms non-policy planning baselines. The algorithm is highly parallelizable, and can run in real time.



\section{Related works}\label{sec:related_work}


Various contingency planning algorithms have been proposed and they can be viewed as different approximations of policy planning. A complete policy planning algorithm should be capable of multi-stage reasoning with bi-directional interactions between the agent and the environment. Since the ego is always reacting to the environment, the concept of bi-directional interaction is also referred to as ego-conditioning, emphasizing on the environment reacting to the ego agent. The application of autonomous driving also asks for high quality trajectories, accurate prediction, interpretability, and scalability. All these features combined makes it difficult to realize a non-compromising policy planning algorithm for autonomous vehicles. As a result, different simplification methods have been proposed. Limited to one stage, \cite{hardy2013contingency} proposed a trajectory optimization method with one trajectory for each scene evolution mode, similar ideas are also seen in \cite{zhan2016non,galceran2017multipolicy} where a predefined set of modes are evaluated online. \cite{cui2021lookout} uses a deep-learned prediction model to generate the modes. \cite{chen2022interactive} performs multistage reasoning via branch MPC and leveraged ego-conditioning, yet requires a simple differentiable prediction model. 

Partially Observed Markov Decision Process (POMDP) ~\cite{bai2015intention,liu2015situation,intentionaware} is a classic policy planning method, yet cannot generate high quality trajectories or use powerful deep-learned prediction models. Game theoretic approaches are well-known for reasoning about bi-directional interactions, yet assume some simple fixed behavior model of the environment, e.g. rational \cite{sadigh2016planning} or noisy Boltzmann \cite{fisac2019hierarchical}. \cite{rhinehart2021contingencies} performs policy planning by training a neural network to react to the environment behavior, yet gives up on multistage reasoning, and is not interpretable and hard to tune. 

Table \ref{table:exist_method} summarizes the various existing methods and their compromises, and we would like to show in the remainder of the paper that \algname{} closes the gap to a practical policy planning method for AV.









%%%%%%%%%%%%%%%%

% \section{Introduction}\label{sec:intro}

% %% Define the problem
% One key challenge of motion planning for autonomous vehicles is handling the interactions with nearby agents, which involves two subproblems, trajectory prediction and motion planning with prediction. The task of trajectory prediction has been studied extensively, ranging from kineamtic models \cite{kong2015kinematic}, maneuver recognition \cite{houenou2013vehicle}, to the various deep learning models that pushed the state-of-the-art in recent years \cite{predictionnet,T++,rhinehart2019precog,ILVM,ScePT}. % These models typically generate mutlimodal predictions and are trained to maximize the likelihood of a dataset of driving logs under the model. 
% A typical planner then uses the prediction result either by considering a single trajectory prediction~\cite{xu2014motion}, multiple trajectory predictions~\cite{cui2021lookout}, or occupancy prediction~\cite{plan_occu,sadat2020perceive}. 

% %% Trajectory vs policy planning
% An important drawback of traditional trajectory planning is that it seeks a single trajectory that performs well under \emph{all} predicted modes of the scene evolution, ignoring the fact that 1) some modes of the future are mutually exclusive and 2) the AV will be able to replan with more information in a future time step. Contingency planning addresses this problem: it generates a motion policy instead of a single trajectory, taking advantage of the prediction model to enumerate possible scene evolution modes and conditioning the ego motion plan on the future scene evolution. 

% %%% Example
% To highlight the difference between a \emph{motion policy} and a single trajectory, consider the scenario depicted on the right end of Fig. \ref{fig:diagram}. The ego vehicle (blue) need to move pass the adjacent vehicle (red). Within the planning horizon the adjacent vehicle either maintains its current lane or cuts in front of the ego vehicle. A non-contingency planner seeks a single trajectory that performs well in both situations and thus will not choose to pass since lane change is a plausible choice for the red vehicle at current time. Alternatively, a contingency motion plan may choose to nudge forward a bit for the first part of the horizon, observe the behavior of the adjacent vehicle, and then decide the subsequent motion. If the red vehicle already started a lane change, the ego vehicle brake to avoid collision; if the red vehicle drives in its own lane, since the ego vehicle is already next to the red vehicle, a sudden lane change is very unlikely, and the ego vehicle can then pass the red vehicle. 





% Prior work on autonomous driving has proposed various contingency planning algorithms. \cite{hardy2013contingency} proposed a trajectory optimization method with one trajectory for each scene evolution mode, similar ideas are also seen in \cite{zhan2016non,galceran2017multipolicy} where a predefined set of modes are evaluated online. \cite{cui2021lookout} uses a deep-learned prediction model to generate the modes, and \cite{chen2022interactive} extends this line of work to include multiple stages via branch MPC and leveraged ego-conditioning. In general, ego-conditioning for optimization-based methods requires a simple differentiable predictive model, which limits the use of sophisticated deep-learning models. Partially Observed Markov Decision Process (POMDP) solvers~\cite{bai2015intention,liu2015situation,intentionaware} are also applied to contingency planning with discretized action spaces. Game theoretic approaches sit on the borderline between contingency planning and traditional motion planning as they leverage the reaction from the environment, yet assume some fixed behavior model of the environment, e.g. rational \cite{sadigh2016planning} or noisy Boltzmann policy \cite{fisac2019hierarchical}, which tend to be uni-modal. In \cite{rhinehart2021contingencies}, contingency planning takes the form of a neural network trained to react to the environment behavior and ego latent, which can incorporate powerful prediction models yet is not interpretable and hard to tune. 

% Unfortunately, despite their various advantages, most of the existing contingency planning algorithms are not ready to be deployed on real-life autonomous vehicles.
% % Multi-node planners optimize over a predefined set of modes~\cite{}. Branch Model Predictive Control (MPC) that performs multi-stage planning with an analytic prediction model.  Partially Observed Markov Decision Process (POMDP) planners  solve a discretized POMDP model for driving. 

% \textit{Desiderata} To meet the requirements of practical autonomous driving, we seek a contingency planning algorithm with the following desired features (1) compatible with state-of-the-art deep-learned predictive models for trajectory forecasting (2) capable of ego-conditioning, i.e., factor in ego vehicle's influence on nearby agents (3) interpretable and easily tunable (4) allow for multistage reasoning that leverages agents' future reactive behavior (5) scale to scenarios with a large number of agents.

% Table \ref{table:exist_method} summarizes some existing contingency planning works and compares them according to our desiderata. 


% In this paper we introduce Tree Policy Planning (\algname{}), a novel sampling-based contingency planning algorithm that jointly fulfills our desiderata for practical autonomous driving. \algname{} consists of three key components: an ego motion sampler, a deep-learned multi-stage prediction model, and a contingency planner that solves for the optimal finite-horizon \emph{motion policy} for the ego vehicle. 

% With a sampling-based approach, we bypass the differentiability constraint and directly apply powerful deep-learning models for ego-conditioned prediction. At the same time, the algorithm stays interpretable and easily tunable. The tree structure extends the one-stage contingency planning to multistage reasoning and greatly increase the allowed complexity of the motion policy. And via parallelization, the seemingly daunting task scales to real-world scenarios and can run in real time.

% We validate our algorithm in closed-loop simulation based on the realistic data-driven traffic model proposed in~\cite{BITS}. Our results show that \algname{} achieves good closed-loop driving performance under real-world scenarios in the nuScenes dataset \cite{nuscenes}, significantly outperforming the benchmarks.


%%%%%%%%%%%%%%%%


% \section{Related Work}


